The Impact of Adversarial Node Placement in Decentralized Federated Learning Networks

As Federated Learning (FL) grows in popularity, new decentralized frameworks are becoming widespread. These frameworks leverage the benefits of decentralized environments to enable fast and energy-efficient inter-device communication. However, this growing popularity also intensifies the need for robust security measures. While existing research has explored various aspects of FL security, the role of adversarial node placement in decentralized networks remains largely unexplored. This paper addresses this gap by analyzing the performance of decentralized FL for various adversarial placement strategies when adversaries can jointly coordinate their placement within a network. We establish two baseline strategies for placing adversarial node: random placement and network centrality-based placement. Building on this foundation, we propose a novel attack algorithm that prioritizes adversarial spread over adversarial centrality by maximizing the average network distance between adversaries. We show that the new attack algorithm significantly impacts key performance metrics such as testing accuracy, outperforming the baseline frameworks by between $9\%$ and $66.5\%$ for the considered setups. Our findings provide valuable insights into the vulnerabilities of decentralized FL systems, setting the stage for future research aimed at developing more secure and robust decentralized FL frameworks.

==> evaluating_cent_measures.tex <==
\subsection{Analysis Setup}\label{sec:analysis_setup}

To analyze the effects of different centrality measures in decentralized setting we considered different types of networks of $n$ devices, which for the purpose of experiments in this section was set to a constant value. The devices communicate with each other via D2D communication, forming a strongly connected, time-invariant directed graph $G = (V, E)$, where each device constitutes a vertex $v_i \in V$ and each existing communication link between any two devices $i, j$ constitutes an edge $e_{ij} := (v_i, v_j) \in E$ in the graph. An edge $e_{ij}$ indicates that the device $i$ can send information to device $j$, and device $j$ can receive that information. Each device has a local private data-set $D_i$, as well as a local loss function $f_i:{\mathbb{R}}^p \rightarrow \mathbb{R}$.

To conduct our analysis, for each network we introduced a set of malicious nodes. These nodes are called adversarial devices, and form a set $A = \{a_1, \ldots, a_m\} \subset V$. Conversely, the set of all non-adversarial devices is defined as  $H = \{h_1, \ldots, h_{n-m}\} = V \setminus A$. Each of the adversarial devices performs a specified malicious attack on their local gradients modifying their resulting local model $x_{i, adv}$. To model the adversarial behavior for our analysis we use the Sybil attack model \cite{lyu2020threats, fung2020mitigating}, where the adversaries follow these standard assumptions:

\textit{Adversarial Assumption 1:} The adversaries can only influence the training process through the aggregation step. The adversaries cannot access or influence the private training and testing data of non-adversarial devices. 

\textit{Adversarial Assumption 2:} The adversaries can change their gradients, data-sets, or any other local variable as well as any information that is being sent out. However, they still participate in the aggregation process similar to honest devices.

\textit{Adversarial Assumption 3:} The adversaries act independently and does not share information with other devices. They all work towards maximizing the loss, but they do not follow any cooperating strategies. 

\textit{Adversarial Assumption 4:} Each adversary has some set attack power $\epsilon$ that they keep constant once the attack starts. 

The specified attack that each adversary launches is considered to be a black box, and as such the attacking nodes can choose any method they see fit that results in the alteration of their local graidents and model. In our symulations to model the adversarial behavior we used the Fast Gradient Sign Method (FGSM) attack \cite{madry2019deep}. 

To participate in the information exchange, each device $v_i \in V$ follows an aggregation scheme of our choosing. There are several frameworks for decentralized aggregation  \cite{6426375, 9825726, 4749425, 5720506, 8267245, doi:10.1137/14096668X, doi:10.1137/16M1084316}, including adversarial robust schemes \cite{6483403}, however for our simulations and centrality measures analysis we decided to use the S-AB aggregation procedure proposed in \cite{9029217}. This scheme incorporates row-stochastic matrices for inter-node model aggregation as well as column-stochastic matrices for gradient estimation, which enables gradient tracking. These properties guarantee that under non-adversarial conditions the devices will all reach consensus and the model reached will be the optimal model assuming that all devices follow the aggregation algorithm.
In this scheme, each device $v_i \in V$ at any given global aggregation time $t \in \mathbb{N}$ has a local model $x_i^{(t)} \in {\mathbb{R}^p}$ that is the estimate of global optimal model $x^*$, and a global gradient estimator vector $y_i^{(t)} \in \mathbb{R}^p$. $x_i^{(0)}$ is initialized randomly for each device, and $y_i^{(0)}$ is initialized as stochastic gradient of the initial model: $g_i(x_i^{(0)}, \zeta_i^{(0)})$, where $\zeta_i{(t)}$ is some batch of data from the $i$-th node local data-set of specified size. Then the exchange of models and gradients proceeds as follows:
\begin{equation*}
    x_i^{(t + 1)} = \underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)}}{d_i^{in}} - \alpha y_i^{(t)}
\end{equation*}
\begin{equation*}
    y_i^{(t + 1)} = \underset{j \in N_i^{in}}{\sum}\frac{y_j^{(t)}}{d_j^{out}} + g_i(x_i^{(t+1)}, \zeta_i^{(t+1)}) - g_i(x_i^{(t)}, \zeta_i^{(t)})
\end{equation*}
where 
\begin{equation*}
    N_i^{in} :=  \{j | (j, i) \in E\} \cup \{i\}
\end{equation*}
\begin{equation*}
    d_i^{in} := |\{j | (j, i) \in E\} \cup \{i\}|
\end{equation*}
\begin{equation*}
    d_i^{out} := |\{j | (i, j) \in E\} \cup \{i\}|
\end{equation*}

Given this setup, the goal of the honest devices is to find a model $x^*$ that minimizes the global loss, as defined in:
\begin{equation} \label{eq:1}
    x^* = \underset{x}{\argmin}f(x) = \underset{x}{\argmin}\underset{i = 1, v_i \in H}{\overset{n-m}{\sum}}f_i(x)
\end{equation}
and the principal goal of the adversarial devices is to either prevent or substantially delay the honest devices from reaching the global optimum by spreading malicious models. We assume the honest nodes do not know about the existence of the adversaries, so from their perspective, the problem becomes:
\begin{equation} \label{eq:2}
    x^* = \underset{x}{\argmin}f(x) = \underset{x}{\argmin}\underset{i = 1}{\overset{n}{\sum}}f_i(x)
\end{equation}

\subsection{Network Setup}\label{sec:network_setup}

We evaluate the effects of different centrality measures on the following network topology types:

\textit{ER Graphs:} In the ER graphs, each directed edge is created with a certain probability $p_{edge} \in [0, 1]$ independently of any other edge and its placement in the network. The ER model is useful in representing randomly created networks, where the inter-node connections do not follow any particular pattern. The ER graphs can model FL processes where there is randomness involved with how the connections are created between different devices, which can be caused by varying availability of devices, randomness in selecting the devices, or mobility of the devices. While ER graphs are not the most common type of graph naturally occurring, due to their random nature they will provide insights into how different centrality measures affect adversarial spread as a base case. 

\textit{Preferential  Attachment Graphs:} The preferential attachment (PA) graphs follow a power-law degree distribution, where a few nodes have a high degree and other nodes have comparably low degrees. During the network formation, the new nodes are attached to existing nodes with a probability proportional to their degree, which results in the emergence of hubs in the network centered around the nodes that were added earlier to the graphs. The PA graph generation property is often observed in many real-world networks, with the primary example being the social networks. Due to their relevance to approximating real-world examples, analyzing PA graphs will provide us with useful insights into implications for the security of FL processes in those networks. 

\textit{Directed Geometric Graphs:} In these types of graphs the nodes are generated in a geometric space, and the edges are created based on the distance between the nodes, in particular if it is below some threshold value. In our experiments we consider randomly generated two-dimensional directed geometric graphs. Geometric graphs can be used to model networks that put emphasis on spacial locations, such as sensor networks, communication networks, or distributed task networks. This results in a plethora of FL networks being modelled by geometric graphs, and analyzing them will give us insight into how the spatial distribution of devices as well as varying communication range affect the adversarial model spread.

\textit{K-out Graphs:} In k-out graphs, each node has $k$ directed outgoing edges connected to other nodes chosen uniformly at random. This property results in a graph with varying in-degrees, but constant out-degrees for each node. These types of graphs can be used in applications where each device interacts with a fixed number of other nodes, regardless of the networks size. Analyzing k-out graphs will give us insight into how the fixed degree of outgoing edges affects the effectiveness of the adversarial model spread.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/ERGraph.png}
         \caption{ER Graph}
         \label{fig:er}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/PAGraph.png}
         \caption{Preferential Attachment Graph}
         \label{fig:pa}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/RGGGraph.png}
         \caption{Random Geometric Graph}
         \label{fig:rg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/KOutGraph.png}
         \caption{k-out Graph}
         \label{fig:kout}
     \end{subfigure}
        \caption{Examples visualizing the synthetically generated graph types}
        \label{fig:graphs}
\end{figure}

Figure 1 illustrates all the types of synthetic graphs that we considered for our analysis. Those types of graphs, were specifically designed and generated to model potential real-world topologies and their behaviors under adversarial conditions. To further our analysis we have also included examples of actual real-world network structures. 


We settled on using the Stanford Large Network Dataset Collection (SNAP) \cite{snapnets}, a dataset that includes many different types of real-world networks. From this collection, we specifically look at networks from the Computer Communication Network category \cite{madani2022dataset}. This category contains networks representing communication strucutres used for connecting computers that run different distributed tasks, which makes them highly relevant to our study of FL frameworks.

By including both the synthetically generated netoworks along with the real-world examples in our analysis, we we hope to create a clear connection between theoretical analysis and practical application, providing insights that can be used in the design of more robust and efficient FL frameworks.

\FloatBarrier

\subsection{Centrality Measures}
Node centrality is a pivotal concept in network analysis that encapsulates the relative significance of the node within the network. There are several various centrality measures that offer distinct insights into node's importance, each with a unique computation procedure and influence. These metrics often exhibit a trade-off where the more comprehensive measures that consider the entire network topology typically require more computational resources, and conversely less computationally demanding matrix may provide a less refined understanding of a node's influence. 

In this paper we explore a range of centrality measures that illustrate the opposing ends of this trade-of. These include in-degree and out-degree centrality, betweenness centrality, closeness centrality, and eigenvector centrality. Each of these provides a unique perspective of a node's influence and place in the network. The following few paragraphs delve into details of each measure. 

Degree centrality is the most basic centrality measure, quantifying number of in-edges and out-edges for in-degree and out-degree centrality measures respectively. It's time complexity is $O(1)$, as each node can keep its degree information at all time without having to perform complex computations.  

Betweenness centrality measures the number of shortest paths from any two nodes that pass through the specified node. It's also the most computationally demanding measure, with a time complexity of $O(|V||E|)$.

Closeness centrality measures the average length of shortest paths from the specified node to all other nodes in the network. Similar to betweenness centrality, its time complexity is $O(|V||E|)$.

Eigenvector centrality is the most mathematical centrality measure of all we considered. This centrality measure calculates the centrality based not only on the influence of specific node but also its neighbor nodes, and all other nodes in the graph, considering the entire network in calculation. The centrality is calculated as $v^TM=\lambda v^T$, where $v^T$ stores the eigenvector centralities for each node in the network, $M$ is an adjacency matrix where $M_{i:j} = 1 \iff (i,j) \in E$, and $\lambda$ is some constant. While the calculation using and adjacency matrix would result in $O(|V|^3)$ time complexity, the power iteration method allows for convergence to the result in $O(|V|)$.


\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{pictures/cent_demo.png}
\caption{Undirected graph with calculated eigenvector centralities for each node. Darker color corresponds to higher centrality.}
\label{fig:cent_demo}
\end{figure}

\FloatBarrier

\subsection{Experimental Setup}
We set up a decentralized training environment to conduct our experiments. Our focus was on small synthetic networks, where the number of nodes was set to 20 for all experiments. The structure of these networks was based on the graph types described in Subsection \ref{sec:network_setup}. For the SNAP dataset, the graphs had a predetermined structure, with the number of nodes varying from 28 to 510. In all cases the malicious nodes were set to be $20\%$ of the total node count, corresponding to four malicious nodes in the synthetic graph scenario.

Each node ran a classification task, training a custom convolutional neural networn on its local data. Subsequently, the model was exchanged according to the aggregation scheme detailed in Subsection \ref{sec:analysis_setup}. We used the FMNIST %and CIFAR10 
data-set for our input data. Each run had two data distribution cases: the IID (Independent and Identically Distributed) case, and the Non-IID. In the IID case, the data was evenly split among all the graph nodes. On the other hand, in the Non-IID case, each node had access to only three classes for training. Accuracy measurements were averaged over 50 runs, with varying seeds and graph realizations of the specified type.

We introduced variability in the graph types by adjusting specific hyperparameters. For Erdős–Rényi (ER) graphs, we varied the connection probability. For Preferential Attachment graphs, we changed the initial cluster size. For Directed Geometric graphs, we adjusted the radius, and for K-Out graphs, we differed the value of $k$.

\subsection{Experimental Results}

The preliminary results of our experiments revealed that the potency of an attack, as determined by the centrality measure, depends on the type of network topology used. Figure \ref{fig:diff_cent_measures_diff_types} illustrates this difference by comparing a Preferential Attachment graph with an ER graph with a connection probability of 0.9.

For the Preferential Attachment graph, we observed negligible differences in attack potency across various centrality measures. However, a clear separation in attack potency was seen in the ER graph. Here, attacks based on In-Degree and Closeness Centrality measures were the most effective, while those based on Eigenvector Centrality were least potent. This observation shows the influence of network type on the effectiveness of different centrality-based attacks.

The analysis for SNAP dataset is applied separately at the end. 

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}  % Adjust width as needed
        \centering
        \includegraphics[width=\textwidth]{pictures/legend_1.png}
        \label{fig:legend_subfig}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.5\textwidth}  % Adjust width as needed
        \centering
        \includegraphics[width=\textwidth]{pictures/pref_attach_graph_c_20_type_dense_2_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{Attack potency for a Preferential Attachment Graph in Non-IID case}
        \label{fig:pref_att_subfig}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.5\textwidth}  % Adjust width as needed
        \centering
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_09_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{Attack potency for an ER Graph in Non-IID case}
        \label{fig:label_for_figure3}
    \end{subfigure}
    
    \caption{Difference between attack potency for different centrality measures between Preferential Attachment Graph and ER Graph}
    \label{fig:diff_cent_measures_diff_types}
\end{figure}

\FloatBarrier

To investigate this relationship, we looked at the properties of the networks that could potentially influence the difference across the centrality measures. We theorized that the observed lack of attack potency difference for various centrality measures could be due to the selection of similar nodes as the most central nodes across these measures.

To validate this hypothesis, we introduced a 'centrality similarity score'. For each centrality measure, we saved its adversarial set, denoted as $A_c$, made of the most central nodes as per that measure. We then evaluated the similarity between these sets across all centrality measures. For any two sets $S_1$ and $S_2$, the similarity score was calculated as $\frac{|S_1 \setminus S_2| + |S_2 \setminus S_1|}{|S_1| + |S_2|}$. The final score was computed by taking a weighted average of the scores for all pairs of different centrality measures. 

This score, normalized between 0 and 1, indicated the similarity between all sets, with 0 corresponding to all sets containing different nodes, and 1 corresponding to all sets being identical. That established score was always evaluated for the adversarial nodes, which also corresponded to the most central nodes for a given measure.

Figure \ref{fig:cent_sim_scores} shows the resulting centrality similarity scores for the corresponding synthetic graph types, calculated for a given percentage of the nodes being adversarial.

\FloatBarrier

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/ER_fmnist.png}
         \label{fig:er_sim}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/pref_attach_fmnist.png}
         \label{fig:pa_sim}
     \end{subfigure}
     \\
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/dir_geom_fmnist.png}
         \label{fig:rg_sim}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{pictures/k_out_fmnist.png}
         \label{fig:kout_sim}
     \end{subfigure}
        \caption{Centrality Similarity Scores for Different Types of Graphs considered.}
        \label{fig:cent_sim_scores}
\end{figure}

\FloatBarrier

The analysis of the centrality similarity scores resulted in insightful observations. As expected, for the adversarial fraction of $1.0$, the similarity scores always had a value of $1$. This is because when all nodes are designated as adversarial the resulting sets are identical across all centrality measures.

However, the graphs showing similarity scores differed significantly across the considered synthetic graph types. While for all types, they show that with higher adversarial fraction, the similarity increases the slopes and offsets of these plots vary significantly. Since for our experiments, we considered the adversarial fraction of $0.2$, we evaluated the scores at that point. 

For ER and K-Out graphs, the similarity scores were relatively low at $0.2$, suggesting that we could expect observable differences in attack potency across different centrality measures for these graph types.

On the other hand, Directed Geometric graphs had moderate similarity scores for graphs with a small radius, and high scores for those with a larger radius. This implied that the differences in attack potency for these graphs would likely be lower than those observed in ER or K-Out graphs.

Finally, Preferential Attachment graphs had high similarity scores for all adversarial fractions. This indicates a high overlap in the sets of most central nodes identified by different centrality measures, which lead us to expect minimal differences in attack potency across various measures for this type of graph.

To validate these expectations, we conducted further accuracy tests for the synthetic graph types. The results of these tests are presented in Figures \ref{fig:er_graph_acc}, \ref{fig:pref_attach_graph_acc}, \ref{fig:dir_geom_graph_acc}, and \ref{fig:kout_graph_acc}, corresponding to the case for ER, Preferential Attachment, Directed Geometric, and K-Out graphs, respectively.

\FloatBarrier
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{pictures/legend_2.png}
        \label{fig:legend}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_01_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{p = 0.1, Non-IID}
        \label{fig:er_graph_acc_1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_01_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{p = 0.1, IID}
        \label{fig:er_graph_acc_2}
    \end{subfigure}
    \\
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_03_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{p = 0.3, Non-IID}
        \label{fig:er_graph_acc_3}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_03_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{p = 0.3, IID}
        \label{fig:er_graph_acc_4}
    \end{subfigure}
    \\
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_05_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{p = 0.5, Non-IID}
        \label{fig:er_graph_acc_5}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_05_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{p = 0.1, IID}
        \label{fig:er_graph_acc_6}
    \end{subfigure}
    \\
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_07_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{p = 0.7, Non-IID}
        \label{fig:er_graph_acc_7}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_07_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{p = 0.7, IID}
        \label{fig:er_graph_acc_8}
    \end{subfigure}
    \\
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_09_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{p = 0.9, Non-IID}
        \label{fig:er_graph_acc_9}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/ER_graph_c_20_p_09_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{p = 0.9, IID}
        \label{fig:er_graph_acc_10}
    \end{subfigure}
    \caption{Testing accuracy with different attacks for various ER graph configurations and data distributions after the attack is deployed.}
    \label{fig:er_graph_acc}
\end{figure}


\FloatBarrier
The analysis of network topologies generated based on the ER graph model revealed observable differences in the performance of various centrality measures. Notably, the distribution of data in the nodes significantly influenced these differences. In the Non-IID case, the differences between the attacks based on different centrality measures were more significant compared to the IID case. Furthermore, these differences were evident across all connection probabilities in the Non-IID case. In the IID case the differences were smaller, but they were more pronounced in for extremely sparse and dense graphs.

When comparing the performance of different centrality measures across different connection probabilities, the closeness centrality and in-degree centrality exhibit better cumulative performance compared to other centrality measures. For sparser graphs where the probability is p = 0.1 or p = 0.3, the betweenness centrality also performs relatively well compared to other measures. The appearance of differences was consistent with our expectations based on the centrality similarity scores.

\FloatBarrier
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{pictures/legend_2.png}
        \label{fig:legend}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/pref_attach_graph_c_20_type_dense_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{Non-IID}
        \label{fig:pref_attach_graph_acc_1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/pref_attach_graph_c_20_type_dense_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{IID}
        \label{fig:pref_attach_graph_acc_2}
    \end{subfigure}
    
    \caption{Testing accuracy with different attacks for Preferential Attachment graphs with different data distributions after the attack is deployed.}
    \label{fig:pref_attach_graph_acc}
\end{figure}
\FloatBarrier

On the other hand, in the case of Preferential Attachment graphs, there were negligible differences the centrality measures performances, as expected based on the centrality similarity scores. This implies that in this graph type, launching an attack on any most central node, irrespective of the centrality measure used, will result in comparable results. Consequently, one conclusion we drew is that if an attacker encounters a network that follows the Preferential Attachment model, they should select either in-degree or out-degree centrality measure to evaluate node centralities for the attack. These measures are the simplest and most computationally efficient, which means they offer an optimal strategy for potential adversaries.

\FloatBarrier
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{pictures/legend_2.png}
        \label{fig:legend}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/dir_geom_graph_c_20_type_2d_close_nodes_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{r = 0.3, Non-IID}
        \label{fig:dir_geom_graph_acc_1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/dir_geom_graph_c_20_type_2d_close_nodes_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{r = 0.3, IID}
        \label{fig:dir_geom_graph_acc_2}
    \end{subfigure}
    \caption{Testing accuracy with different attacks for Directed Geometric graphs with different data distributions after the attack is deployed.}
    \label{fig:dir_geom_graph_acc}
\end{figure}
\FloatBarrier

In the case of Directed Geometric graphs, there exist differences between centrality measures, however they are not as pronounced as in the ER graphs. This again aligns with what we expected based on the centrality similarity scores. While no specific centrality measure has a significantly better performance than the others, both out-degree and in-degree centrality measures exhibit strong performance in both IID and Non-IID cases. This suggests that in an adversarial scenario, these measures could be used to identify the most central nodes to atack.

\FloatBarrier
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{pictures/legend_2.png}
        \label{fig:legend}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/k_out_graph_c_20_k_5_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{k = 5, Non-IID}
        \label{fig:kout_graph_acc_1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/k_out_graph_c_20_k_5_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{k = 5, IID}
        \label{fig:kout_graph_acc_2}
    \end{subfigure}
    \\
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/k_out_graph_c_20_k_10_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_non_iid.png}
        \caption{k = 10, Non-IID}
        \label{fig:kout_graph_acc_1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{pictures/k_out_graph_c_20_k_10_acc_atk_FGSM_advs_4_adv_pow_100_atk_time_25_iid_type_iid.png}
        \caption{k = 10, IID}
        \label{fig:kout_graph_acc_2}
    \end{subfigure}
    \caption{Testing accuracy with different attacks for various K-Out graph configurations and data distributions after the attack is deployed.}
    \label{fig:kout_graph_acc}
\end{figure}
\FloatBarrier

For the last synthetic graph type, the K-Out graphs, the differences between the centrality measures are again more significant, aligning with the expectation from the centralities similarity score. Across all scenarios, the in-degree centrality demonstrated good performance, with the closeness centrality exhibiting marginally better performance for higher values of k. This suggest that the closeness centrality might be the best measure to use if the computation time is not a concern, especially for higher k values. 

\FloatBarrier
Our experiments involving the \textbf{SNAP dataset} posed some challenges due to the inherent difference in the number of nodes and the custom  topology of each network. A key problem that we encountered was the lack of a requirement for the graphs to be strongly connected. This meant that the information from some nodes may never spread throughout the entire network, which undermines one of the fundamental assumptions of our analysis. This property resulted in a high variance in the averaged honest accuracy, even for smaller networks, as can be seen in Figure \ref{fig:SNAP_ex_acc}. This has prevented us from being able to draw meaningful conclusions for the SNAP dataset case, and investigating improvements to this setup is one of the future directions for this research.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\textwidth]{pictures/SNAP_Cisco_c_28_type_g20_acc_atk_FGSM_advs_5_adv_pow_100_atk_time_25_iid_type_iid.png}
\caption{Testing accuracy with different attacks for a SNAP dataset 28-client graph, IID.}
\label{fig:SNAP_ex_acc}
\end{figure}
\FloatBarrier

% add all centrality data

% New direction -> How about proposing a centrality based attack that is more potent based on node centrality in the network

% Check this idea: See if maybe attacking nodes based on one centrality, but analyzing the rate based on another leads anywhere
% Another thought: What if we could use that defense, but also tune the value f based on the centrality of the given node in the network, such that it minimizes the error?
% Here is the new direction idea. Either analyze how attacking the central nodes affects the potency of the attack and epidemic spread, OR analyze/propose new attack framework on how given a certain centrality we can attack it. 
% Add a section with paragraph for each type of graph + snap dataset

==> theory.tex <==
After experiments how it supports the results
In our experiments, the potency of attacks based on eigenvector centrality measure consistently matched or fell short of the performance of the most effective centrality measures for each network type. Consequently, we decided to analyze the theoretical convergence rate bound for eigenvector centrality. This analysis could provide insights into the minimum performance that can be experimentally expected from the most effective centrality measures.

To conduct our analysis, we first establish the following standard assumptions:

\textit{Assumption 1:} Each node has a local loss function $f_i(.)$ that is $\mu$-strongly-convex, i.e., $\forall i \in \mathbb{N}$  s.t. $v_i \in V$ and $\forall \mathbf{x}, \mathbf{y} \in \mathbb{R}^p$  there exists a constant $\mu$ such that:
\begin{equation}\label{assumption_1}
    \left(\nabla f_i(\mathbf{x})-\nabla f_i(\mathbf{y})\right)^{\top}(\mathbf{x}-\mathbf{y}) \geq \mu\|\mathbf{x}-\mathbf{y}\|^2
\end{equation}

\textit{Assumption 2:} Each node has a local loss function $f_i(.)$ that is $\beta$-smooth, i.e., $\forall i \in \mathbb{N}$  s.t. $v_i \in V$ and $\forall \mathbf{x}, \mathbf{y} \in \mathbb{R}^p$ there exists a constant $\beta$ such that 
\begin{equation}\label{assumption_2}
    \left\|\nabla f_i(\mathbf{x})-\nabla f_i(\mathbf{y})\right\| \leq \beta \|\mathbf{x} - \mathbf{y}\|
\end{equation}

\textit{Assumption 3:} The Stochastic Gradient (SG) associated with each node is unbiased and has a bounded variance i.e., $\forall i \in \mathbb{N}$ s.t. $v_i \in V$ and $\forall \mathbf{x} \in \mathbb{R}^p$ we have $\mathbb{E}\left[\widetilde{\nabla} f_i(\mathbf{x})-\nabla f_i(\mathbf{x}) \mid \mathbf{x}\right]=0$, and there exists a constant $\varrho > 0$ such that $\mathbb{E}\left\|\widetilde{\nabla} f_i(\mathbf{x})-\nabla f_i(\mathbf{x})\right\|^2 \leq \varrho^2$


Given these assumptions, let a given node $v_i \in V$ have a model $x_i^{(t)} \in \mathbb{R}^p$ at time $t \in \mathbb{N}$. We will conduct the analysis assuming each node $i$ uses a standard consensus-only based aggregation algorithm: 
\begin{equation*}
    x_i^{(t+1)} = \underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)}}{d_i^{in}} - \alpha \widetilde{\nabla} f_i(x_i^{(t)})
\end{equation*}

We can represent that equation in a matrix form:
\begin{equation*}
    X(t+1) = MX(t) - \alpha \Delta(t)
\end{equation*}
Where $X(t) = [x_1^{(t)}, x_2^{(t)}, \cdots, x_{|V|}^{(t)}]^T$, $M$ is a row-stochastic adjacency matrix representing the graph $G$ that the nodes form, where the entry $m_{i,j} := \frac{1}{d_i^{in}}$ if $j \in N_i^{in}$ and $0$ otherwise, and $\Delta(t) = [\widetilde{\nabla} f_1(x_1^{(t)}), \widetilde{\nabla} f_2(x_2^{(t)}), \cdots, \widetilde{\nabla} f_{|V|}(x_{|V|}^{(t)})]^T$.

By the Perron-Frobenius theorem we know that $\mathbf{1}$ is the only right eigenvector of $M$. Next, let $\mathbf{v}^T$ represent the transpose of left principal eigenvector of $M$, which also corresponds to a vector of eigenvector centralities for the nodes in graph $G$, i.e. the $i$-th entry of $\mathbf{v}$: $v_i$ is the eigenvector centrality of client $i$. Notice that:
\begin{gather*}
    \mathbf{v}^TX(t+1) = \mathbf{v}^T(AX(t) - \alpha\Delta(t)) \\
    =  \mathbf{v}^TAX(t) - \alpha \mathbf{v}^T\Delta(t) = \mathbf{v}^TX(t) - \alpha \mathbf{v}^T\Delta(t)
\end{gather*}
So we find that:
\begin{equation}\label{eig_cent_eq}
    \mathbf{v}^TX(t+1) = \mathbf{v}^TX(t) - \alpha \mathbf{v}^T\Delta(t)
\end{equation}

Next, for our analysis we introduce $X^*$, which contains optimal models for each node, and $\hat{X}(t)$, which is the equivalent of $X(t)$ in a situation where every node in the network is an honest node. 

We will consider the value of optimality gap $(X(t) - X^*) - (\hat{X}(t) - X^*) = X(t) - \hat{X}(t)$ in our analysis. It compares the difference between the node models in the presence of adversaries to the node models when all nodes are honest.

Finally, we assume that the adversarial clients will always keep their stochastic gradients above a threshold value $\delta_{adv,min}$, in a way that will prevent the honest clients from ever reaching an optimal point.

Consider the value of $\mathbb{E}||X(t+1) - \hat{X}(t+1)||_F^2$. It follows that:
\begin{gather*}
    \mathbb{E}||(X(t+1) - \hat{X}(t+1))||_F^2  \\ \geq \underset{\mathbf{w}:\|\mathbf{w}\|_2 = 1}{\max}
    \mathbb{E}||\mathbf{w}^T(X(t+1) - \hat{X}(t+1))||_2^2  \\ \geq
     \mathbb{E}||\mathbf{v}^T(X(t+1) - \hat{X}(t+1))||_2^2\\ 
    = \mathbb{E}||\mathbf{v}^T((AX(t) - \alpha \Delta(t)) - (A\hat{X}(t) - \alpha \hat{\Delta}(t)))||_2^2 \\
    = \mathbb{E}||\mathbf{v}^T((AX(t) - A\hat{X}(t)) - \mathbf{v}^T\alpha (\Delta(t) - \hat{\Delta}(t))||_2^2 \\
    \overset{(a)}{=} \mathbb{E}||\mathbf{v}^T((X(t) - \hat{X}(t)) - \mathbf{v}^T\alpha (\Delta(t) - \hat{\Delta}(t))||_2^2 \\
    =  \mathbb{E}||\mathbf{v}^T((X(0) - \hat{X}(0)) - \underset{i = 0}{\overset{t}{\sum}}\mathbf{v}^T\alpha (\Delta(i) - \hat{\Delta}(i))||_2^2 \\
    \overset{(b)}{=} \mathbb{E}||\underset{i = 0}{\overset{t}{\sum}}\mathbf{v}^T\alpha (\Delta(i) - \hat{\Delta}(i))||_2^2 \\
    = {\alpha}^2\mathbb{E}||\mathbf{v}^T \underset{i = 0}{\overset{t}{\sum}}(\Delta(i) - \hat{\Delta}(i))||_2^2 \\
    = {\alpha}^2\mathbb{E}||\underset{j \in A}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\widetilde{\nabla} f_j(x_j^{(i)}) - \widetilde{\nabla}\hat{f_j}(x_j^{(i)})) + \\ \underset{j \in H}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\widetilde{\nabla} f_j(x_j^{(i)}) - \widetilde{\nabla}\hat{f_j}(x_j^{(i)}))||_2^2 \\
    \overset{(c)}{=}  {\alpha}^2\mathbb{E}||\underset{j \in A}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\delta_{adv,min} - \widetilde{\nabla}\hat{f_j}(x_j^{(i)})) + \\ \underset{j \in H}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\widetilde{\nabla} f_j(x_j^{(i)}) - \widetilde{\nabla}\hat{f_j}(x_j^{(i)}))||_2^2 \\
    \geq {\alpha}^2\mathbb{E}||\underset{j \in A}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\delta_{adv,min} - \widetilde{\nabla}\hat{f_j}(x_j^{(i)}))||_2^2 - \\|| \underset{j \in H}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\widetilde{\nabla} f_j(x_j^{(i)}) - \widetilde{\nabla}\hat{f_j}(x_j^{(i)}))||_2^2
\end{gather*}
where:

%- (a) follows from \ref{eig_cent_eq}.

%- (b) follows from the assumption that the initial models for case with malicious agents and without them are the same.

%- (c) follows from the assumption about the lower bounded gradients on adversarial clients.

%Therefore the final expression is:
%\begin{equation}\label{eq_bound}
%\begin{split}
%    \mathbb{E}||\mathbf{v}^T(X(t+1) - \hat{X}(t+1))||_F^2 \\
%    {\geq}  {\alpha}^2\mathbb{E}||\underset{j \in A}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\delta_{adv,min} - \widetilde{\nabla}\hat{f_j}(x_j^{(i)})) + \\ \underset{j \in H}{\sum}v_j\underset{i = 0}{\overset{t}{\sum}}(\widetilde{\nabla} f_j(x_j^{(i)}) - \widetilde{\nabla}\hat{f_j}(x_j^{(i)}))||_F^2
%\end{split}
%\end{equation}

%This expression provides a lower bound on the convex combination of differences between the models in adversarial and honest environments. This bound has two key parts: the eigenvector centralities of the adversarial clients and their gradient bound (as shown in the first part of the expression on the right), and the honest client centralities and the cumulative gradient difference (as indicated in the second part of the expression on the right).

%The cumulative gradient difference can be represented by a positive constant that is a function of the number of adversaries and $\delta_{adv,min}$. This is the result of fact that in the adversarial scenario, the malicious models perpetually maintain the honest gradients above a certain minimum threshold, as they never converge to an optimal model.

%While this bound provides us with valuable insights, a further more detailed investigation into the aforementioned constant, along with empirical validation of the result, will improve our understanding of the dynamics of the explored relationship.


%By the Perron-Frobenius theorem we know that $\mathbf{1}$ is the only right eigenvector of $A$. Next, by $(3)$:
%\begin{equation}
%    \mathbf{v}^T\mathbf{x}^{(t + 1)} =  \mathbf{v}^TA \mathbf{x}^{(t)} -  \mathbf{v}^T\alpha  \mathbf{y}^{(t)}
%\end{equation}
%where $\mathbf{v}$ is the left principal eigenvector of $A$ that also corresponds to the eigenvector centralities of each client $i$ in the graph $G$, i.e. the $i$-th entry of $\mathbf{v} = v_i$ is the eigenvector centrality of client $i$.
%Next:
%\begin{equation}
%    \mathbf{v}^T\mathbf{x}^{(t + 1)} = \mathbf{v}^TA \mathbf{x}^{(t)} -  \mathbf{v}^T\alpha  %\mathbf{y}^{(t)} = 
%    \mathbf{v}^T \mathbf{x}^{(t)} -  \mathbf{v}^T\alpha  \mathbf{y}^{(t)}
%\end{equation}
%Rewriting that we get:
%\begin{equation}
%    \mathbf{v}^T(\mathbf{x}^{(t + 1)} - \mathbf{x}^{(t)}) =  -  \alpha\mathbf{v}^T\mathbf{y}^{(t)}
%\end{equation}
%Then:
%\begin{gather*}
%     \mathbb{E}||\mathbf{x}^{(t + 1)}-\mathbf{x}^{(t)}||_2^2  = \\
%\end{gather*}

%In the distributed hypothesis learning we have: 
%$x_i^{(t + 1)} = \underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)}}{d_i^{in}} - \alpha g(x(t), \zeta) $
% Assume that the attack has been happening for some time - analyze the most general time instance. 2 cases - attack hasn't occured so far (the original paper case), assume the attack takes place at some t_a, also t - t_a >= n - 1. 
% Log agents belief -> local gradients, then can show that the aggregation is the same as the hypothesis testing rule
%\begin{gather*}
%     \mathbb{E}||x_i^{(t+1)}-x_i^{(t)}||_2^2 \\ 
 %    = \mathbb{E}||\underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)}}{d_j^{in}} - \alpha y_i^{(t)}-x_i^{(t)}||_2^2 \\ 
  %   = \mathbb{E}||\underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)}}{d_i^{in}} - \alpha y_i^{(t)}- \frac{d_i^{in}}{d_i^{in}} x_i^{(t)}||_2^2 \\
  %   = \mathbb{E}||\underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)} - x_i^{(t)}}{d_i^{in}} - \alpha y_i^{(t)}||_2^2 \\
  %   = \mathbb{E}[(\underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)} - x_i^{(t)}}{d_i^{in}} - \alpha y_i^{(t)})^T(\underset{j \in N_i^{in}}{\sum}\frac{x_j^{(t)} - x_i^{(t)}}{d_i^{in}} - \alpha y_i^{(t)})] \\
%\end{gather*}

%\begin{gather*}
%    E||v^T((x(t+1)-x^*) -(\hat{x}(t+1) - x^*))||_F^2 \\
%    = E||v^T(x(t+1) - \hat{x}(t+1))||_F^2 \\
%    = E||v^T(Ax(t) - \alpha g_{adv}(t) -A\hat{x}(t) - \alpha g(t))||_F^2 \\
%    = E||v^TAx(t) - v^T\alpha g_{adv}(t) - v^TA\hat{x}(t) + v^T\alpha g(t)||_F^2 \\
%    = E||v^T(x(t) - \hat{x}(t)) - v^T\alpha(g_{adv}(t) - g(t)) ||_F^2 \\
%    = E||v^T(x(0)-\hat{x}(0)) - \underset{i = 1}{\overset{t}{\sum}}v^T\alpha(g_{adv}(i) - g(i))||_F^2 \\ 
%    = \alpha^2 E||\underset{i = 1}{\overset{t}{\sum}}v^T(g_{adv}(i) - g(i))||_F^2 \\
%    = \alpha^2 E||v^T(\underset{i = 1}{\overset{t}{\sum}}g_{adv}(i) - \underset{i = 1}{\overset{t}{\sum}}g(i))||_F^2 \\
%    \geq \alpha^2 E||v^T(\underset{i = 1}{\overset{t}{\sum}}g_{adv,min} - \underset{i = 1}{\overset{t}{\sum}}g(i))||_F^2 \\
%    = \alpha^2 E||v^Ttg_{adv,min} - v^T\underset{i = 1}{\overset{t}{\sum}}g(i)||_F^2 \\
%    \geq \alpha^2 E||v^Ttg_{adv,min} - v^T\underset{i = 1}{\overset{t}{\sum}}g(0)||_F^2 \\
%    = \alpha^2t^2 E||v^T(g_{adv,min} - g(0))||_F^2
%\end{gather*}


%Expectations of honest client diffs will be 0, but expectations of now will differ and change over time. Use centrality measure here to evaluate that. Although that depends on when the attack was used. Maybe consider induction

% Revisit top-k notion -> check the notion about the tradeoff between the centralities of many nodes and the distance between those nodes (don't choose 2 close most central nodes, instead try to have high distance between 2 relatively central nodes). Try to come up with an algorithm that combines the centrality-distance tradeoff to select which nodes to attack in the network. Assume the adversary know the whole topology of the network (adversary knows everything).
% Consider instead of graph distances we attack based on the model divergence (how different the models are, so most central node + node that has most dissimilar model from the- most central node).
% Consider some other combinations of the centality - ... tradeoff to see which combination provides best results (maybe include a comparison in the paper between the different strategies). 
% Finish the proofs with the value for the delta value
